Sounding Board: A User-Centric and Content-Driven Social Chatbot

We present Sounding Board, a social chatbot that won the 2017 Amazon Alexa Prize. The system architecture consists of several components including spoken language processing, dialogue management, language generation, and content management, with emphasis on user-centric and content-driven design. We also share insights gained from large-scale online logs based on 160,000 conversations with real-world users.

==> sections/intro.tex <==

Engaging in long-term contentful and coherent conversation has been a longstanding challenge in AI. 
% Many existing chatbots such as Eliza \cite{Weizenbaum1996Comm}, Parry
% \cite{Colby1975AI}, and Alice \cite{Wallace2009ALICE} support mostly superficial
% engagements.
% Conversational assistants in commercial products such as Amazon Alexa, Microsoft
% Cortana,  Google Assistant, and Apple Siri, are more contentful, but focus on
% short, goal-oriented interactions.
% While variants of Recurrent Neural Networks (RNNs) have proven successful across many NLP tasks \cite{wu2016google,yang2017breaking,suzuki2017cutting}, several recent works have reported that neural network based models have difficulties generating conversations with long-term coherence \citep{serban2017hierarchical,sato2017modeling,shao2017generating,tian2017make,knowledge-grounded-neural-conversation-model}.
Unlike earlier systems such as Eliza \cite{Weizenbaum1996Comm}, Parry
\cite{Colby1975AI}, and Alice \cite{Wallace2009ALICE}, recent work  has sought to use massive, dynamic online content to engage users.
Conversational assistants in commercial products such as Amazon Alexa, Microsoft
Cortana, Google Assistant, and Apple Siri, are capable of using online content,
but focus on short, task-oriented interactions.
While variants of recurrent neural networks have proven successful across
many NLP tasks \cite{wu2016google,suzuki2017cutting,Yang2018ICLR}, recent findings indicate that neural network based models have difficulties
generating conversations with long-term coherence
\citep{serban2017hierarchical,sato2017modeling,shao2017generating,tian2017make,Ghazvininejad2018AAAI}.


The Alexa Prize sets forth a new challenge: creating a system that can hold a
coherent and engaging conversation 
%with humans 
on current events and popular topics such as sports,
politics, entertainment, fashion and technology
%for 20 minutes. 
\cite{AlexaPrize2017}.
%With this definition in mind, we developed
%Toward this goal, our system 
Our system, {Sounding Board},\footnote{\url{https://sounding-board.github.io}}
demonstrates that it is feasible to build an agent that can engage in long-term conversation when backed by rich content and knowledge of the user obtained through interaction.
%Sounding Board addresses this challenge by modeling conversations based on the rich collection of content it updates daily from online sources, and adapting the conversation based on its knowledge of the user.
Our system won the inaugural Amazon Alexa 
Prize with an average score of 3.17 on a 5-point scale  and an average conversation duration of 10:22, evaluated by a panel of independent judges.\footnote{\url{https://developer.amazon.com/alexaprize/2017-alexa-prize}}

% \begin{figure}[t]
% 	\centering 
% 	%trim={<left> <lower> <right> <upper>}
% 	\includegraphics[width=0.48\textwidth]{figs/convoExample.png}
% 	\caption{Sample conversation between a user (U) and Sounding Board (S). 
% 		Note that the user utterances may contain speech recognition errors.}
% 	\label{fig:sample_convo}
% \end{figure}

\begin{figure}[t]
	\centering 
	%trim={<left> <lower> <right> <upper>}
	\vspace{-4mm}
	\includegraphics[width=0.46\textwidth,trim=2cm 9cm 3.5cm 1cm]{figs/sample_dialog_larger.pdf}
	\caption{A sample dialog. 
	Suspected speech recognition errors in the user utterances are underlined.}
	\label{fig:sample_convo}
\end{figure}

\begin{comment}
\begin{table}[]
\centering
\caption{A sample dialog. 
	Suspected speech recognition errors in the user utterances are underlined.}
\label{tab:sample_convo}
\begin{tabular}{|c|l|l|}
\hline
\textbf{Turn} & \multicolumn{1}{c|}{\textbf{User}} & \multicolumn{1}{c|}{\textbf{Sounding Board}} \\ \hline
1 & Let's chat & Hi! This is an Alexa Prize socialbot. How's your day? \\ \hline
2 & I'm five. & \begin{tabular}[c]{@{}l@{}}Glad to hear it! We could talk about robots, batman,\\ or superman. Say "next", to chat about other things.\end{tabular} \\ \hline
3 & Superman. & \begin{tabular}[c]{@{}l@{}}It looks like you wanna chat about superman. \\ I was high up in the cloud when I realized: \\ If people don't recognize Clark Kent as Superman \\ because of his glasses, does his eye doctor know \\ his true identity?\end{tabular} \\ \hline
4 & I guess so. & \begin{tabular}[c]{@{}l@{}}Did you know that Henry Cavill almost missed the \\ call for the role of Superman cause he was playing \\ "World of Warcraft"?\end{tabular} \\ \hline
5 & \begin{tabular}[c]{@{}l@{}}Really, I didn't \\ know that.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Weird, right? Speaking of superman, Did you see: \\ Superman? It was released in 1997. It's a comedy.\end{tabular} \\ \hline
6 & \begin{tabular}[c]{@{}l@{}}Yes, it was \\ hilarious.\end{tabular} & \begin{tabular}[c]{@{}l@{}}I'm glad you feel this is hilarious. Which part do \\ you like best about this movie?\end{tabular} \\ \hline
7 & \begin{tabular}[c]{@{}l@{}}The part when \\ he met \\ lewis leah.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Interesting. Meccartin, and raffi co-directed this film. \\ The movie has a 6.3 out of 10 on IMDB. which \\ seems pretty good! do you like the movie's director?\end{tabular} \\ \hline
\end{tabular}
\end{table}
\end{comment}

%We approached the open-ended problem posed in the challenge by focusing on two core 
%We focus on two core 
%issues: how do we cater the conversation to a %individual 
%user and how do we provide content that is interesting and relevant to the
%conversation?
There are two key design objectives of Sounding Board: to be \emph{user-centric} and \emph{content-driven}. 
% the current topic of 
Our system is \textit{user-centric} in that 
%users choose the topics they wish to discuss and can change them at any time. 
users can control the topic of conversation, while the system adapts responses to the user's likely interests by gauging the user's personality.
%and incorporates that knowledge in recommending topics that are more likely to engage the user.
%to better adapt the conversation topics to the user's likely interests. 
% We also learn personality information about the user and incorporate that knowledge 
% into the way we design the conversation.\eclark{The personality part should be
% more specific. e.g., ``...incorporate that knowledge to recommend topics'', etc.}
Sounding Board is also \emph{content-driven}, as it continually supplies interesting and relevant information to continue the conversation, enabled by a rich content collection that it updates daily.
%The system can guide the conversation and recommend topics based on the information it has access to.
%In this way, the system can drive the conversation forward and cover a wide breadth of topics.
It is this content that can engage users for a long period of time and drive the conversation forward. A sample conversation log is shown in Figure~\ref{fig:sample_convo}. 
% \noah{the figure's text is soooo tiny}

%The approach we used to build Sounding Board is described in \S\ref{sec:system_arch}, followed by a discussion in \S\ref{sec:insights} about the strengths and weaknesses of the approach based on analyses of conversation logs collected with Amazon Alexa users. Finally, \S\ref{sec:conclusion} summarizes the main features of the system.

We describe the system architecture in \S\ref{sec:system_arch}, share our insights based on  large scale conversation logs in \S\ref{sec:insights}, and conclude in \S\ref{sec:conclusion}.

